Applications of $\alpha$-strongly regular distributions to Bayesian auctions

Two classes of distributions that are widely used in the analysis of Bayesian auctions are the Monotone Hazard Rate (MHR) and Regular distributions. They can both be characterized in terms of the rate of change of the associated virtual value functions: for MHR distributions the condition is that for values $v < v'$, $\phi(v') - \phi(v) \ge v' - v$, and for regular distributions, $\phi(v') - \phi(v) \ge 0$. Cole and Roughgarden introduced the interpolating class of $\alpha$-Strongly Regular distributions ($\alpha$-SR distributions for short), for which $\phi(v') - \phi(v) \ge \alpha(v' - v)$, for $0 \le \alpha \le 1$. In this paper, we investigate five distinct auction settings for which good expected revenue bounds are known when the bidders' valuations are given by MHR distributions. In every case, we show that these bounds degrade gracefully when extended to $\alpha$-SR distributions. For four of these settings, the auction mechanism requires knowledge of these distribution(s) (in the other setting, the distributions are needed only to ensure good bounds on the expected revenue). In these cases we also investigate what happens when the distributions are known only approximately via samples, specifically how to modify the mechanisms so that they remain effective and how the expected revenue depends on the number of samples.

==> app-sampling-prelim.tex <==

\section{Missing Results and Proofs from Section~\ref{sec:sampling}}

\begin{proof}[\textbf{Lemma~\ref{empreserve}}]
We assume that the statement in Lemma~\ref{empquantrange} holds, which it does with probability $1-\delta$.  By Lemma~\ref{empquantrange}, \[\CR(\overline{r}) = q(\overline{r})\overline{r} \geq \frac{1}{(1+\gamma)^2}\overline{q}(\overline{r})\overline{r} = \frac{1}{(1+\gamma)^2}\overline{\CR}(\overline{r}). \numberthis \label{emp}\]  At this point we consider two cases, $\overline{q}(r) \geq \xi$ and $\overline{q}(r) < \xi$.

\noindent\textbf{Case 1:} $\overline{q}(r) \geq \xi$

By the definition of $\overline{r}$, $\overline{\CR}(\overline{r}) \geq \overline{\CR}(r)$ and therefore~\eqref{emp} is bounded below by $\frac{1}{(1+\gamma)^2}\overline{\CR}(r)$. We use Lemma~\ref{empquantrange} again to see that \[\frac{1}{(1+\gamma)^2}\overline{\CR}(r) = \frac{1}{(1+\gamma)^2} \overline{q}(r)r \geq \frac{1}{(1+\gamma)^4}q(r)r = \frac{1}{(1+\gamma)^4}\CR(r).\]

\noindent\textbf{Case 2:} $\overline{q}(r) < \xi$

By the definition of $\overline{r}$, $\overline{\CR}(\overline{r}) \geq \overline{\CR}(\overline{q}(\overline{v}(\xi)))$ and therefore~\eqref{emp} is bounded below by $\frac{1}{(1+\gamma)^2}\overline{\CR}(\overline{q}(\overline{v}(\xi)))$.  We use Lemma~\ref{empquantrange} again to see that \[\frac{1}{(1+\gamma)^2}\overline{\CR}(\overline{q}(\overline{v}(\xi))) = \frac{1}{(1+\gamma)^2}\overline{q}(\overline{v}(\xi))\overline{v}(\xi) \geq \frac{1}{(1+\gamma)^4}q(\overline{v}(\xi))\overline{v}(\xi)  = \frac{1}{(1+\gamma)^4}\CR(\overline{v}(\xi)).\]  Because $\CR$ is convex and by assumption $\overline{v}(\xi) < r$, it follows that \[\frac{1}{(1+\gamma)^4}\CR(\overline{v}(\xi)) \geq \frac{1-q(\overline{v}(\xi))}{(1+\gamma)^4}\CR(r).\]  Finally, by Lemma~\ref{empquantrange}, $q(\overline{v}(\xi)) \leq \overline{q}(\overline{v}(\xi))(1+\gamma)^2$ and therefore we obtain a final bound of $\frac{1-\xi(1+\gamma)^2}{(1+\gamma)^4}\CR(r)$ as desired.
\end{proof}

\begin{proof}[\textbf{Lemma~\ref{empquant}}]
The upper bound on $\overline{\CR}(\overline{q})$ follows from Lemma 6.3 in~\cite{CR1}.  To prove the lower bound, we choose $j$ so that $t_{j+1} = \frac{2(j+1)-1}{2m} \geq \overline{q} \geq \frac{2j-1}{2m} = t_j$.  As defined in~\cite{CR1}, the values $t_i$ denote the empirical quantiles of the samples.    As stated in~\cite{CR1}, $t_j(1+\gamma) \geq t_{j+1}$.  If $\overline{q} \leq \overline{q}(\overline{r})$, then, \begin{align*}
\overline{\CR}(\overline{q}) \geq \overline{\CR}(t_j) &\geq t_j v(t_j(1+\gamma)^2) \tag{by Lemma 6.3 in~\cite{CR1}} \\
&\geq \frac{\overline{q}}{(1+\gamma)} v(\overline{q}(1+\gamma)^2) \\
&= \frac{1}{(1+\gamma)^3}\CR(\overline{q}(1+\gamma)^2).
\end{align*}  Otherwise, if $\overline{q} \geq \overline{q}(\overline{r})$, then, \begin{align*}
\overline{\CR}(\overline{q}) \geq \overline{\CR}(t_{j+1}) &\geq t_{j+1} v(t_{j+1}(1+\gamma)^2) \tag{by Lemma 6.3 in~\cite{CR1}} \\
&\geq \overline{q} v(\overline{q}(1+\gamma)^3) \\
&= \frac{1}{(1+\gamma)^3}\CR(\overline{q}(1+\gamma)^3).
\end{align*}
\end{proof}

\hide{In order to use Lemma~\ref{empquant} to compare the empirical revenue curve with the actual one, we use the following lemma from~\cite{CR1}.}

\hide{\begin{lem}\label{valuequant}
Let $F$ be a regular distribution.  Let $q(r) \geq q_1 \geq q_2$, where $q(r)$ is the quantile of the reserve price for $F$.  Then $v(q_2) \leq \frac{q_1}{q_2}v(q_1)$.
\end{lem}
\begin{proof} % [Lemma~\ref{valuequant}]
$\phi(q) \geq 0$ for $q \leq q(r)$, and consequently $R(q_1) \geq R(q_2)$.  $R(q_1) = q_1\cdot v(q_1)$ and $R(q_2) = q_2\cdot v(q_2)$.  Thus $q_1 \cdot v(q_1) \geq q_2\cdot v(q_2)$, and the result follows.
\end{proof}}

%Using the above bound in Lemma~\ref{empquant} yields the following corollary.

\hide{\begin{cor}\label{empquantc}
Conditioned on $\mathcal{E}_a$, for all empirical quantiles $q(r) \geq \overline{q} \geq \xi$, 
%\frac{1}{(1+\gamma)^2}\CR(\overline{q}) \leq 
\[\overline{\CR}(\overline{q}) \leq \CR(\overline{q})(1+\gamma)^2.\]
\end{cor}}

\hide{The following lemma, a slight modification of a claim in~\cite{CR}, upper bounds the revenue curve for quantiles less than $q(r)$.  This will allow us to lower bound $q(\overline{r})$.

\begin{lem}\label{reserveb}
Let $F$ be an $\alpha$-SR distribution with \skr{reserve} price $r$.  For $q \leq q(r)$ and $0 < \alpha < 1$, \[\CR(q) \leq \CR(q(r)) \frac{1}{1-\alpha}\left( \left(\frac{q}{q(r)}\right)^{\alpha}-\alpha\frac{q}{q(r)}\right).\]
\end{lem}
\begin{proof}By letting $q_0 = r$ in Lemma 6.3 from~\cite{CR} and using the fact that $q(r)/f(r) = r$, it follows that \[v(q) \leq r+\frac{r}{1-\alpha}\left[\left(\frac{q(r)}{q}\right)^{1-\alpha}-1\right].\]   \begin{align*}\CR(q) &= q\cdot v(q) \\
&\leq qr+q\frac{r}{1-\alpha}\left[\left(\frac{q(r)}{q}\right)^{1-\alpha}-1\right] \\
&= \CR(q(r))\frac{q}{q(r)}\left[1+\frac{\left(\frac{q(r)}{q}\right)^{1-\alpha}-1}{1-\alpha}\right] \\
&= \CR(q(r))\frac{1}{1-\alpha}\left( \left(\frac{q}{q(r)}\right)^{\alpha}-\alpha\frac{q}{q(r)}\right).\end{align*} 
\end{proof}

\hide{\begin{lem}
Let $F$ be an $\alpha$-SR distribution with monopoly price $r$.  For $q_1 \leq q_2 \leq q(r)$ and $0 < \alpha < 1$, \[CR(q_1) \leq CR(q_2)\frac{1}{1-\alpha}\left(\frac{q_1}{q_2}\right)^{\alpha}.\]
\end{lem}}

\hide{We note that the original lemma was proved in the case $q_2 = q(r)$.  However, the proof still holds in the case $q_2 \leq q(r)$.}

The following lemma lower bounds the quantile of the empirical reserve price in terms of the quantile of the actual reserve price.

\begin{lem}\label{reservequant}
Let $0 < \alpha \leq 1$, and let $F$ be an $\alpha$-SR distribution.  Then conditioned on $\mathcal{E}_a$, \[q(\overline{r}) \geq \left(1-\sqrt{\frac{8\gamma}{\alpha}}\right) q(r).\]
\end{lem}
\begin{proof} % [Lemma~\ref{reservequant}]
If $q(\overline{r}) \ge q(r)$ the result holds trivially; so for the rest of the proof, we will assume that $\overline r > r$.
To simplify the presentation, we let $s = \sqrt{8\gamma/\alpha}$.
Now assume for the sake of a contradiction that the statement of the lemma does not hold.  
We show that this implies that \skr{$\overline{CR}(r) \geq \overline{CR}(\overline{r})$} which contradicts the choice of $\overline{r}$.

By \skr{Lemma~\ref{empquantrange}}, as $\overline r > r$, \skr{$\overline{CR}(\overline{r}) \leq CR(\overline{r}) (1+\gamma)^2$}.   
Thus
%
%By our assumption on $g(\overline{r})$, we can apply Lemma~\ref{reserveb} to get a strict upper bound of 
%
\begin{align*}
CR(q(\overline{r}))(1+\gamma)^2 &< CR\left( (1-s) q(r) \right) (1+\gamma)^2 \\
&\leq CR(q(r))\frac{1}{1-\alpha}\left((1-s)^{\alpha}-\alpha(1-s)\right)(1+\gamma)^2 \numberthis \label{qbound}\\
&\hspace*{2in} \mbox{(by Lemma~\ref{reserveb}).}
\end{align*}  
The Taylor expansion of $(1-s)^{\alpha}$ is $\sum_{i=0}^{\infty} \frac{(-1)^is^{i}\alpha(\alpha-1)\cdots(\alpha-i+1)}{i!}$. 
It follows that $(1-s)^{\alpha} \leq 1-\alpha s - (1-\alpha)\alpha s^2/2$, as $s < 1$.
Therefore~\eqref{qbound} is bounded above by 
\[CR(q(r))\frac{1}{1-\alpha}\left(1-\alpha- (1-\alpha)\frac{\alpha s^2}{2}\right)(1+\gamma)^2 = CR(q(r))\left(1-\frac{\alpha s^2}{2} \right) (1+\gamma)^2\numberthis \label{qboundtwo}.\]  
On replacing $s$ with $\sqrt{8\gamma/\alpha}$ in~\eqref{qboundtwo} this becomes \[CR(q(r))(1-4\gamma)(1+\gamma)^2 \leq \frac{1}{(1+\gamma)^2}CR(q(r)),~~ \mbox{as $1-4\gamma \leq 1/(1+\gamma)^4$.}\]

%By our assumption, $q(\overline{r}) \leq q(r)$, and we can use Lemma~\ref{reserveb} to get a strict upper bound of \[CR(r)(1+\gamma)^2\frac{1}{1-\alpha}\left(\left(\frac{1-\alpha}{(1+\gamma)^4}\right)^{1/\alpha}\right)^{\alpha} = \frac{CR(r)}{(1+\gamma)^2}.\]  ]

By \skr{Lemma~\ref{empquantrange}} again, this is bounded above by \skr{$\overline{CR}(r)$}, reaching a contradiction.
\end{proof}}

==> properties.tex <==

\section{Properties of $\alpha$-SR regular distributions}~\label{property}

We now prove some properties of $\alpha$-SR regular distributions that generalize analogous properties
of MHR distributions, and that will be helpful in extending revenue bounds
that have previously only been shown to apply to MHR distributions.

% The first result, given in~\cite{CR}, is a lower bound on the probability that some valuation taken from $F$ is greater than the monopoly price $r$.

\begin{lem}\label{reservebound}[\cite{CR}]
Let $F$ be an $\alpha$-SR regular distribution with monopoly price $r$.
%
% \item If $\alpha = 1$, then $1-F(r) \geq \frac{1}{e}$.
%
If $0 < \alpha < 1$, then $1-F(r) \geq \alpha^{1/(1-\alpha)}$.
\end{lem}

\hide{
The next result bounds values $v$ from above in terms of the monopoly price $r$ and the virtual valuation $\phi(\alpha)$. (It generalizes Lemma 3.1 in~\cite{HR} from the case $\alpha = 1$.)

\begin{lem}\label{reservevirtualbound}
Let $\alpha \geq 0$ and let $F$ be an $\alpha$-SR regular distribution with monopoly price $r$ and virtual valuation function $\phi$.  Then, if $v \geq r$, \[r+\frac{\phi(v)}{\alpha} \geq v.\]
\end{lem}


\begin{proof}
By definition, as $\phi$ is $\alpha$-SR regular, $\phi(v)-\phi(r) \geq \alpha(v-r)$.
Because $r$ is the monopoly price, $\phi(r) = 0$; thus $\phi(v) \geq \alpha(v-r)$.
Solving for $v$ gives the above inequality.
\end{proof}
}

\hide{
The following lemma gives a lower bound on $h(v)$ that will be used later.

\begin{lem}\label{hbound}
Let $0 \leq \alpha \leq 1$ and let $F$ be an $\alpha$-SR regular distribution with virtual valuation function $\phi$.  Then for all $v_1 \leq v_2$, \[h(v_2) \geq \frac{1}{(1-\alpha)(v_2-v_1)+1/h(v_1)}.\]
% where $h(v) = f(v)/(1-F(v))$.
\end{lem}

\begin{proof}
When $\alpha = 1$, this states that $h(v_2) \geq h(v_1)$ which is by definition in this case.

By definition, as $\phi$ is $\alpha$-SR regular, \[\phi(v_2)-\phi(v_1) \geq \alpha(v_2-v_1).\]  Substituting $\phi(v) = v-1/h(v)$ yields \[-\frac{1}{h(v_2)} \geq (\alpha-1)(v_2-v_1)-\frac{1}{h(v_1)}.\]  On multiplying both sides by $-1$ and taking their reciprocals we obtain the desired inequality.
\end{proof}
}

\hide{
Using almost the same proof as above, we obtain the following upper bound on $h(v)$.  This was also given in~\cite{CR} for the special case of $v_2 = r$.

\begin{lem}\label{hbound2}
Let $0 \leq \alpha \leq 1$ and let $F$ be an $\alpha$-SR regular distribution with virtual valuation function $\phi$.  Then for all $v_1 \leq v_2$ such that $1/h(v_2)-(1-\alpha)(v_2-v_1) > 0$, \[h(v_1) \leq \frac{1}{1/h(v_2)-(1-\alpha)(v_2-v_1)}.\]
% where $h(v) = f(v)/(1-F(v))$.
\end{lem}

\begin{proof}
Again, when $\alpha = 1$, this states that $h(v_1) \leq h(v_2)$.

As in the proof of Lemma~\ref{hbound}, \[\frac{1}{h(v_1)} \geq (\alpha-1)(v_2-v_1)+\frac{1}{h(v_2)}.\]  Note that the left-hand side is always positive, while there are no restrictions on the right-hand side.  If the right-hand side is not positive, then we do not have a useful bound on $h(v_1)$.  If the right-hand side is positive, i.e. if $1/h(v_2)-(1-\alpha)(v_2-v_1) > 0$, we can take the reciprocal of both sides to get the desired inequality.
\end{proof}
}

\hide{
Note that the condition $1/h(v_2)-(1-\alpha)(v_2-v_1) > 0$ holds in the case that $v_2 = r$, where $r$ is the reserve price, as $1/h(r) = r$. In addition, Lemmas~\ref{hbound} and~\ref{hbound2} hold in the case that $F$ is defined on the set $\{1, \ldots, L\}$, using the same proof.

We can also give a lower bound on the probability that $\phi(v) > \alpha v/2$.  This is helpful when we want to only consider the case that $\phi(v)$ is bounded away from $0$.

\begin{lem}\label{div2}
Let $0 < \alpha < 1$ and let $F$ be an $\alpha$-SR regular distribution, with monopoly price $r$ and virtual valuation function $\phi$.  Then \[\Pr_{v \sim F} [\phi(v) > \alpha v/2 ] \geq \left(\frac{\alpha}{2-\alpha}\right)^{1/(1-\alpha)}.\]
\end{lem}

\begin{proof}
$\phi(v) > \alpha v/2$ if and only if \[\phi(v) - \alpha v > - \frac{\alpha v}{2}.\]  As $\phi$ is $\alpha$-SR regular, the left-hand side is non-decreasing, while the right-hand side is decreasing. Therefore, there exists some $k^*$ such that the inequality holds if and only if $v >  k^*$; $k^*$ is given by $\phi(k^*)-\alpha k^* = -(\alpha k^*)/2$.

As $\phi(k^*) = k^* - 1/h(k^*)$, it follows that \[h(k^*) = \frac{2}{(2-\alpha) k^*}. \numberthis \label{intersect}\]  Now \begin{align*}1/h(k^*)-(1-\alpha)(k^*-v) &= (2-\alpha)k^*/2-(1-\alpha)(k^*-v )\\
&= \alpha/2 k^*+(1-\alpha)v \\
&\geq 0.\end{align*}  Then when $v \leq k^*$, Lemma~\ref{hbound2} can be used with $v_1 = v$ and $v_2 = k^*$, yielding \[h(v) \leq \frac{1}{(1-\alpha)(v-k^*)+(2-\alpha) k^* / 2}.\] Therefore,

\begin{align*}
H(k^*) = \int_0^{k^*} h(v) dv
&\leq \int_0^{k^*} \frac{1}{(1-\alpha)(v-k^*)+(2-\alpha) k^* / 2} dv \\
&= \frac{1}{1-\alpha}\log((1-\alpha)(v-k^*)+(2-\alpha) k^* / 2)  \biggr|_0^{k^*}\\
&= \frac{1}{1-\alpha} \log\left(\frac{(2-\alpha) k^* / 2}{(2-\alpha) k^* / 2 -(1-\alpha) k^*}\right) \\
&= \frac{1}{1-\alpha} \log\left(\frac{2-\alpha}{\alpha}\right).
\end{align*}

Finally, by the definition of $k^*$,
\begin{align*}
\Pr_{v \sim F} [\phi(v) > \alpha v/2 ] &= \Pr_{v \sim F} [v > k^*] \\
& = e^{- H(k^*) dv} \\
&\geq e^{\frac{1}{1-\alpha} \log\left(\frac{2-\alpha}{\alpha}\right)} \\
&= \left(\frac{2-\alpha}{\alpha}\right)^{-1/(1-\alpha)}.
\end{align*} The first equality comes from the fact that $1-F(v) = e^{-H(v)}$.  The inequality comes from the upper bound on $h(v)$ given above.
\end{proof}
}

The following lemma extends Lemma 3.10 in~\cite{DRY} to $\alpha$-SR regular distributions.
% As a corollary, we are also able to upper bound the expected valuation as a function of $\alpha$ and the reserve price.

\begin{lem}\label{welfare}
Let $0 < \alpha < 1$ and let $F$ be an $\alpha$-SR distribution, with monopoly price $r$ and revenue function $\hat{R}$.  Let $V(t)$ denote the expected welfare of a single-item auction with a posted price of t and a single bidder with valuation drawn from $F$. For every non-negative number $t \geq 0$, \[\hat{R}(\max\{t, r\}) \geq \alpha^{1/(1-\alpha)} V(t).\]
\end{lem}
\hide{
\begin{proof}
As in the proof of this lemma for MHR distributions, we split this into two cases, $t \leq r$ and $t \geq r$.

In both cases, we can write the left-hand side as $s \cdot (1-F(s)) = s\cdot e^{-H(s)}$, where $H(v) = \int_0^{v} h(v)$, and $s = \max\{t, r\}$.

\noindent\textbf{Case 1}: $t \leq r$.

We start from the fact that \[V(t) \leq \int_0^{\infty} e^{-H(v)}dv.\]  As shown in Lemma 3.10 in~\cite{DRY}, this only uses the fact that $h$ is non-negative, and therefore still applies for the case of $\alpha$-SR regular distributions.

In order to upper bound $V(t)$, we start by lower bounding $H(v)$.  Because $h(v)$ is always non-negative, $H(v)$ is always non-negative.  When $v \leq r$, this will be the only lower bound we use.  Otherwise, we will use the lower bound for $h(v)$ from Lemma~\ref{hbound} when $v \geq r$ to lower bound $H(v)$ when $v \geq r$.  In particular, if $v \geq r$, then

\begin{align*}
H(v) &= \int_0^v h(v)dv \\
&= \int_0^r h(v)dv + \int_r^v h(v)dv \\
&= H(r)+ \int_r^v h(v)dv \\
&\geq H(r) + \int_r^v \frac{1}{(1-\alpha)(v-r)+r}dv \tag{by Lemma~\ref{hbound}}\\
&= H(r)+ \frac{1}{1-\alpha}\log\left((1-\alpha)v+\alpha r\right) \biggr|_r^v \\
&=  H(r) + \frac{1}{1-\alpha}\log\left((1-\alpha)\frac{v}{r}+\alpha)\right).
\end{align*}

Therefore,

\begin{align*}
V(t) &\leq \int_0^{\infty} e^{-H(v)}dv \\
&= \int_0^{r} e^{-H(v)}dv + \int_r^{\infty} e^{-H(v)}dv \\
&\leq \int_0^{r} e^{-H(v)}dv+ e^{-H(r)}\int_r^{\infty} e^{-\frac{1}{1-\alpha}\log((1-\alpha)\frac{v}{r}+\alpha))}dv \\
&= \int_0^{r} e^{-H(v)}dv + e^{-H(r)}\int_r^{\infty} ((1-\alpha)\frac{v}{r}+\alpha)^{1/(\alpha-1)} dv \\
&= \int_0^{r} e^{-H(v)}dv +e^{-H(r)} \frac{\alpha-1}{\alpha} \cdot \frac{r}{1-\alpha} \cdot \left(\frac{1-\alpha}{r}v+\alpha\right)^{\alpha/(\alpha-1)} \Biggr|_r^{\infty} \\
&= \int_0^{r} e^{-H(v)}dv - e^{-H(r)}\frac{r}{\alpha} \left(\frac{1-\alpha}{r}v+\alpha\right)^{\alpha/(\alpha-1)} \Biggr|_r^{\infty} \\
&= \int_0^{r} e^{-H(v)}dv+ e^{-H(r)}\frac{r}{\alpha} \numberthis \label{Vbound}
\end{align*}

We rewrite this as \[ \left(\int_0^{r} e^{-H(v)}dv+e^{-H(r)}\frac{r}{\alpha}\right) e^{-H(r)} e^{H(r)}.\]  In the case that $t \leq r$, $\max\{r, t\} = r$.  In order to upper bound this, we consider $e^{H(r)} \int_0^{r} e^{-H(v)}dv$ by itself.  Note that by Lemma~\ref{hbound2}, if $v \leq r$, \[h(v) \leq \frac{1}{(1-\alpha)(v-r)+r}.\]  It follows that

\begin{align*}
H(r)-H(v) &= \int_v^r h(v)dv \\
&\leq \int_v^r \frac{1}{(1-\alpha)(v-r)+r}dv \\
&= \frac{1}{1-\alpha}\log\left((1-\alpha)v+\alpha r\right) \biggr |_v^r \\
&=  \frac{1}{1-\alpha}\log\left(\frac{r}{(1-\alpha)v+\alpha r}\right).
\end{align*}

Therefore,

\begin{align*}
e^{H(r)} \int_0^{r} e^{-H(v)}dv &\leq \int_0^r e^{\frac{1}{1-\alpha}\log\left(\frac{r}{(1-\alpha)v+\alpha r}\right)}dv \\
&= \int_0^r \left(\frac{(1-\alpha)v}{r}+\alpha \right)^{1/(\alpha-1)}dv \\
&=  - \frac{r}{\alpha} \left(\frac{1-\alpha}{r}v+\alpha\right)^{\alpha/(\alpha-1)} \Biggr|_0^{r} \\
&= \frac{r}{\alpha}\left(\alpha^{\alpha/(\alpha-1)}-1\right).
\end{align*}

Plugging this into our bound for $V(t)$ yields

\begin{align*}
V(t) &\leq  \left(\frac{r}{\alpha}\left(\alpha^{\alpha/(\alpha-1)}-1\right)+\frac{r}{\alpha}\right)e^{-H(s)} \tag{recall that $r = s$}\\
&=  \alpha^{1/(\alpha-1)} \cdot s \cdot e^{-H(s)} \\
&= \hat{R}(s) \alpha^{1/(\alpha-1)}, \tag{as $\hat{R}(s) = se^{-H(s)}$}
\end{align*}  and therefore, $\hat{R}(\max\{t, r\}) \geq \alpha^{1/(1-\alpha)} V(t)$ as desired.

\vspace{3mm}

\noindent\textbf{Case 2:} $t \geq r$.

From the proof of Lemma 3.10 in~\cite{DRY}, \[V(t) = e^{-H(t)} \cdot \left[ t + \int_t^{\infty} e^{-(H(v)-H(t)) } dv\right].\]  By Lemma~\ref{hbound}, for all $v \geq t$,

\begin{align*}
H(v)-H(t) &= \int_t^v h(v)dv \\
&\geq \int_t^v \frac{1}{(1-\alpha)(v-r)+r}dv  \tag{by Lemma~\ref{hbound}} \\
&= \frac{1}{1-\alpha}\log\left((1-\alpha)v+\alpha r\right) \biggr|_t^v \\
&=  \frac{1}{1-\alpha}\log\left(\frac{(1-\alpha)v+\alpha r} {(1-\alpha)t+\alpha r}\right).
\end{align*}

Therefore,

\begin{align*}
\int_t^{\infty} e^{-(H(v)-H(t)) } dv &\leq \int_t^{\infty} e^{\frac{-1}{1-\alpha}\log\left(\frac{(1-\alpha)v+\alpha r} {(1-\alpha)t+\alpha r}\right)}dv \\
&= \int_t^{\infty} \left(\frac{(1-\alpha)v+\alpha r} {(1-\alpha)t+\alpha r}\right) ^ {1 / (\alpha -1) }dv \\
&= \frac{\alpha-1}{\alpha} \cdot \frac{(1-\alpha)t+\alpha r}{1-\alpha} \cdot \left(\frac{(1-\alpha)v+\alpha r} {(1-\alpha)t+\alpha r}\right) ^ {\alpha / (\alpha -1) } \Biggr|_t^{\infty} \\
&= \frac{(1-\alpha)t+\alpha r}{\alpha} \\
& \leq \frac{t}{\alpha}.
\end{align*}

It follows that

\begin{align*}
V(t) &= e^{-H(t)} \cdot \left[ t + \int_t^{\infty} e^{-(H(v)-H(t)) } dv\right] \\
&\leq e^{-H(t)} \cdot \left[ t + \frac{t}{\alpha} \right ] \\
&= e^{-H(t)} \cdot t \cdot \left(\frac{\alpha+1}{\alpha}\right) \\
&\leq e^{-H(t)} \cdot t \cdot\alpha^{1/(\alpha-1)}.
\end{align*}

The last inequality comes from the fact that for $0 < \alpha < 1$, $(\alpha+1)/\alpha \leq \alpha^{1/(\alpha-1)}$.  This is true if and only if $(\alpha+1)^{\alpha-1} \leq \alpha^{\alpha}$.  Because $0 < \alpha < 1$, the left-hand side is at most $1$, and the right-hand side is at least $1$.
\end{proof}
}

\hide{
In addition, we can show % ~\eqref{Vbound} yields
the following corollary.

\begin{cor}\label{expected}
Let $0 < \alpha \leq 1$ and let $F$ be an $\alpha$-SR regular distribution with monopoly price $r$.  Then \[V(0) = \mathbb{E}[v] = \int_0^{\infty} (1-F(v))dv \leq r\left(1+\frac{1}{\alpha}\right).\]
\end{cor}

\begin{proof}
\textbf{Case 1:} $\alpha = 1$.

Because $H$ is convex, when $v \geq r$, \[H(v) \geq H(r)+h(r)(v-r).\]  Because $h(r) = 1/r$, \[H(v) \geq H(r) + \frac{v-r}{r}.\]  Therefore
\begin{align*}
\int_0^{\infty} (1-F(v))dv &= \int_0^{r} (1-F(v))dv+\int_r^{\infty} (1-F(v))dv \\
&= \int_0^{r} (1-F(v))dv+\int_r^{\infty} e^{-H(v)}dv \\
&\leq r+\int_r^{\infty} e^{-H(r) - (v-r)/r}dv \\
&= r+e^{-H(r)}r \\
&\leq 2r
\end{align*} as desired.

\vspace{3mm}

\noindent \textbf{Case 2:} $\alpha < 1$.

Because $\mathbb{E}[v] = V(0)$, we can upper-bound $e^{-H(v)}$ in~\eqref{Vbound} by $1$ for all $v$, as $H(v)$ must always be positive.  Doing this yields the desired result.
\end{proof}
}

\hide{
We note that except for Corollary~\ref{expected}, all of the above lemmas are tight in the case of the worst-case distributions $F^{\alpha}$. Corollary~\ref{expected} is tight in the case of the worst-case distribution $F^{\alpha}$, but slightly modified so that a point mass is placed at the reserve price $r$ and no element of the support is smaller than $r$.  The following lemma~\cite{CR} is also tight in the worst-case distribution $F^{\alpha}$.  This fact will be used to prove additional results about $\alpha$-SR regular distributions.

\begin{lem}~\label{densitybound}
Let $F$ be an $\alpha$-SR regular distribution, and let $f$ be the density function for $v$.  Let $q_0 \in [0, 1]$.  Then for $q \leq q_0$, \[f(q) \geq f(q_0)\left(\frac{q}{q_0}\right)^{2-\alpha}.\]
\end{lem}

\begin{proof}
Recall that $\phi(v) = v-q(v)/f(v)$ and $\frac{dv}{dq} = -1/f(v)$.  Hence $\frac{d\phi}{dq} = \frac{-2}{f(v)}+\frac{q(v)}{f(v)^2}\frac{df}{dq}$.  And the condition $\frac{d\phi}{dv} \geq \alpha$ amounts to $\frac{d\phi}{dq} \leq \frac{-\alpha}{f(v)}$.  Thus $\frac{q(v)}{f(v)^2}\frac{df}{dq} \leq \frac{2-\alpha}{f(v)}$ or $\frac{d}{dq}\ln{f} \leq \frac{1}{q}(2-\alpha)$.  For $q \leq q_0$, this yields $f(q) \geq f(q_0)\left(\frac{q}{q_0}\right)^{2-\alpha}$ as desired.
\end{proof}
}

\hide{
We use Lemma~\ref{densitybound} to prove the following result about the cumulative distribution function of $\alpha$-SR regular distributions.

\begin{lem}\label{cdfbound}
Let $F$ be an $\alpha$-SR regular distribution, and let $F^{\alpha}$ be an $\alpha$-SR regular distribution such that $f(q) = f(q_0)\left(\frac{q}{q_0}\right)^{2-\alpha}$ for all $q_0 \in [0, 1]$ and $q \leq q_0$. If for some $v_0$, $F(v_0) > F^{\alpha}(v_0)$, then $F(v) \geq F^{\alpha}(v)$ for all $v \geq v_0$.
\end{lem}

\begin{proof}
Assume that the statement of the lemma is not true.  We will show that this leads to a contradiction.  In particular, assume that there are $v_1$ and $v_2$ with $v_2 > v_1$, $F(v_1) > F^{\alpha}(v_1)$, but $F(v_2) < F^{\alpha}(v_2)$.  Then there must exist $v_3$, with $v_1 < v_3 < v_2,$ such that the function $F(v)-F^{\alpha}(v)$ crosses the $x$-axis from above at $v = v_3$.  It follows that $f(v_3)- f^{\alpha}(v_3) < 0,$ where $f$ and $f^{\alpha}$ are the density functions, or derivatives, of $F$ and $F^{\alpha}$ respectively.

Suppose that the function $F(v)-F^{\alpha}(v)$ crosses the $x$-axis from below at $v_0 < v_1$.  If no such $v_0$ exists, let $v_0 = 0$.  Then it follows that $f(v_0)-f^{\alpha}(v_0) \geq 0$.  This is true even if $v_0 = 0$, as in this case, for all $v$ in the interval $[v_0, v_1]$ it holds that $F(v)-F^{\alpha}(v) \geq 0$.

Let $q(v)$ be the quantile of $v$ in $F$, and let $q^{\alpha}(v)$ be the quantile of $v$ in $F^{\alpha}$.  Note that $q(v_0) = q^{\alpha}(v_0)$ and $q(v_3) = q^{\alpha}(v_3)$.  By Lemma~\ref{densitybound}, for all $v \geq v_0$, \[f(v) \geq f(v_0)\left(\frac{q(v)}{q(v_0)}\right)^{2-\alpha}.\]  Because $f(v_0) \geq f^{\alpha}(v_0)$ and $q(v_0) = q^{\alpha}(v_0)$, the above is bounded below by \[f^{\alpha}(v_0)\left(\frac{q(v)}{q^{\alpha}(v_0)}\right)^{2-\alpha}.\]  On setting $v = v_3$, as $q(v_3) = q^{\alpha}(v_3),$ we obtain the bound \[f(v_3) \geq f^{\alpha}(v_0)\left(\frac{q^{\alpha}(v_3)}{q^{\alpha}(v_0)}\right)^{2-\alpha}.\]  However, the right-hand side is equal to $f^{\alpha}(v_3)$, which contradicts the statement that $f(v_3)- f^{\alpha}(v_3) < 0$.
\end{proof}
}

\hide{
\begin{lem} \label{square}
Let $0 < \alpha < 1$ and let $F$ be an $\alpha$-SR regular distribution.  Then, \[ \frac{\alpha}{1+\alpha} \int_0^{\infty} (1-F(v))dv \leq \int_0^{\infty} (1-F(v))^2dv.\]
\end{lem}

\begin{proof}
We start by defining the distribution $G$ as \[G(v) = F\left(v\cdot \left(\int_0^{\infty} (1-F(v))dv\right)^{-1}\right).\]  Note that $G$ is also $\alpha$-SR regular, and that \[\frac{\int_0^{\infty} (1-G(v))dv}{\int_0^{\infty} (1-G(v))^2dv} = \frac{\int_0^{\infty} (1-F(v))dv}{\int_0^{\infty} (1-F(v))^2dv}.\]  Therefore proving the lemma for $G$ implies the lemma for $F$.

Let $G^{\alpha}$ be defined analogously with respect to the worst case distribution $F^{\alpha}$.  The distribution $G^{\alpha}$ satisfies the inequality in the lemma, and therefore it is enough to prove that \[\frac{\int_0^{\infty} (1-G(v))dv}{\int_0^{\infty} (1-G(v))^2dv} \leq \frac{\int_0^{\infty} (1-G^{\alpha}(v))dv}{\int_0^{\infty} (1-G^{\alpha}(v))^2dv}.\]  Both $G$ and $G^{\alpha}$ are normalized so that $\int_0^{\infty} (1-G(v))dv = \int_0^{\infty} (1-G^{\alpha}(v))dv = 1$, and therefore it is enough to show that \[\int_0^{\infty} (1-G(v))^2dv \geq \int_0^{\infty} (1-G^{\alpha}(v))^2dv.\]

We apply Lemma~\ref{cdfbound} to $G$ and $G^{\alpha}$.  Because $G^{\alpha}$ is the normalized version of the worst case distribution, the conditions of Lemma~\ref{cdfbound} hold.  It follows that there exists a $v_0$ such that $G(v) \geq G^{\alpha}(v)$ when $v \geq v_0$, and $G(v) \leq G^{\alpha}(v)$ when $v < v_0$.

We now show that \[\int_0^{\infty} (1-G(v))^2dv-\int_0^{\infty} (1-G^{\alpha}(v))^2dv \geq 0.\]  We rewrite this as \[\int_0^{\infty} ((1-G(v))-(1-G^{\alpha}(v)))((1-G(v))+(1-G^{\alpha}(v)))dv.\]  Because $\int_0^{\infty} (1-G(v))-(1-G^{\alpha}(v))dv = 0$, it follows that \[\int_0^{v_0} (1-G(v))-(1-G^{\alpha}(v))dv = -\int_{v_0}^{\infty} (1-G(v))-(1-G^{\alpha}(v))dv.\]  Finally, because both $1-G$ and $1-G^{\alpha}$ are decreasing functions and because $((1-G(v))-(1-G^{\alpha}(v))) \leq 0$ when $v \geq v_0$ and $((1-G(v))-(1-G^{\alpha}(v))) \geq 0$ when $v < v_0$, it follows that \begin{multline*}
\int_0^{\infty} ((1-G(v))-(1-G^{\alpha}(v)))((1-G(v))+(1-G^{\alpha}(v)))dv \geq \\
((1-G(v_0))+(1-G^{\alpha}(v_0)))\left(\int_0^{\infty} ((1-G(v))-(1-G^{\alpha}(v)))dv\right) \geq 0\end{multline*} as desired.
\end{proof}
}

%\begin{lem} \label{square}
%Let $0 < \alpha < 1$ and let $F$ be an $\alpha$-SR regular distribution.  Then, \[ \frac{\alpha^2}{(1+\alpha)^2} \left(1-\alpha^{\frac{1+\alpha}{1-\alpha}}\right) \int_0^{\infty} e^{-H(v)}dv \leq \int_0^{\infty} e^{-2H(v)}dv.\]
%\end{lem}
%\begin{proof}
%We start by lower bounding the right-hand side.  Consider all $v \leq r$.  By Lemma~\ref{hbound2}, \[h(v) \leq \frac{1}{(1-\alpha)(v-r)+r}.\]

%It follows that when $v \leq r$,

%\begin{align*}
%H(v) &= \int_0^{v} h(v)dv \\
%&\leq \int_0^{v} \frac{1}{(1-\alpha)(v-r)+r}dv \\
%&= \frac{1}{1-\alpha} \log((1-\alpha)(v-r)+r) \Biggr|_0^v \\
%&= \frac{1}{1-\alpha}\log\left(\frac{(1-\alpha)(v-r)+r}{\alpha r}\right).
%\end{align*}

%Therefore,


%\begin{align*}
%\int_0^{\infty} e^{-2H(v)}dv &\geq \int_0^{r} e^{-2H(v)}dv \\
%&\geq \int_0^{r} e^{\frac{-2}{1-\alpha}\log\left(\frac{(1-\alpha)(v-r)+r}{\alpha r}\right)}dv \\
%&= \int_0^{r} \left(\frac{(1-\alpha)(v-r)+r}{\alpha r}\right)^{\frac{-2}{1-\alpha}}dv \\
%&= \frac{1-\alpha}{-1-\alpha} \cdot \frac{\alpha r}{1- \alpha} \cdot \left(\frac{(1-\alpha)(v-r)+r}{\alpha r}\right)^{\frac{-1-\alpha}{1-\alpha}} \Biggr|_0^r \\
%&= \frac{\alpha r}{1+\alpha}\cdot \left(1-\alpha^{\frac{1+\alpha}{1-\alpha}}\right).
%\end{align*}

%Additionally, by Corollary~\ref{expected}, \[\int_0^{\infty} e^{-H(v)}dv = \int_0^{\infty} (1-F(v))dv \leq r \left(1 + \frac{1}{\alpha}\right) = r \left(\frac{\alpha+1}{\alpha}\right),\] which proves the lemma.
%\end{proof}

\hide{
We note that as $\alpha$ approaches $1$, the ratio $\int_0^{\infty} e^{-2H(v)}dv / \int_0^{\infty} e^{-H(v)}dv$ is bounded below by $0.5$.  An analog of this result for $\alpha = 1$ is shown in the proof of Lemma 4.1 in~\cite{HR}; in this case  $\int_0^{\infty} e^{-2H(v)}dv / \int_0^{\infty} e^{-H(v)}dv \geq 0.5.$  Lemma~\ref{square} can be used to prove the following lemma.

\begin{lem}\label{minmax}
Let $0 < \alpha < 1$ and let $F$ be an $\alpha$-SR regular distribution.  Then, \[\mathbb{E}_{v_1, v_1 \sim F}[\max\{v_1, v_2\}] \leq \left(\frac{2+\alpha}{\alpha}\right)\mathbb{E}_{v_1, v_1 \sim F}[\min\{v_1, v_2\}].\]
\end{lem}

\begin{proof}
Note that \[\mathbb{E}_{v_1, v_1 \sim F}[\max\{v_1, v_2\}] = \int_0^{\infty} 1-F(x)F(x)dx.\] This can be seen by noting that $\Pr[\max\{v_1, v_2\} \leq x] = 1-F(x)F(x)$.  In addition, \[\mathbb{E}_{v_1, v_1 \sim F}[\min\{v_1, v_2\}] =  \int_0^{\infty} (1-F(x))(1-F(x))dx\] as $\Pr[\min\{v_1, v_2\} \leq x] = (1-F(x))(1-F(x)).$  Therefore,  \begin{multline*}\frac{\mathbb{E}_{v_1, v_1 \sim F}[\max\{v_1, v_2\}] }{\mathbb{E}_{v_1, v_1 \sim F}[\min\{v_1, v_2\}]} = \frac{\int_0^{\infty} 1-F(x)F(x)dx}{\int_0^{\infty} (1-F(x))(1-F(x)) dx} = \\ \frac{\int_0^{\infty} 2(1-F(x))- (1-F(x))^2 dx}{\int_0^{\infty} (1-F(x))^2 dx} = \frac{2\int_0^{\infty} (1-F(x)) dx}{\int_0^{\infty} (1-F(x))^2 dx}-1.\end{multline*}

By Lemma~\ref{square}, this is bounded above by \[\left(\frac{2(1+\alpha)}{\alpha}-1\right) = \frac{2+\alpha}{\alpha}\] as desired.
\end{proof}


Lemma~\ref{minmax} can be generalized to condition on the event that $\max\{v_1, v_2\} \geq t$ for any constant $t$.  This generalizes Lemma 4.1 in~\cite{CR} from the case $\alpha = 1$.
}

\begin{lem}\label{conditioned}
Let $0 < \alpha < 1$ and let $F$ be an $\alpha$-SR regular distribution, and $\phi$ be its virtual valuation function.
Then, for all $t$,
\begin{align*}
&\mathbb{E}_{v_1, v_1 \sim F}[\max\{v_1, v_2\} | \max\{v_1, v_2\} \geq t] \leq \\
&~~~~~~~~~\left(\frac{2+\alpha}{\alpha}\right)\mathbb{E}_{v_1, v_1 \sim F}[\max(\phi(v_1), \phi(v_2)) | \max\{v_1, v_2\} \geq t].
\end{align*}
\end{lem}
\hide{
\begin{proof}
First, note that we can replace $\min\{v_1, v_2\}$ in Lemma~\ref{minmax} with $\max(\phi(v_1), \phi(v_2))$, as Myerson's Lemma shows that the two are equal in expectation~\cite{M}.  By Lemma~\ref{minmax}, this corollary holds when $t = 0$.

Let $C(\alpha) = \left(\frac{2+\alpha}{\alpha}\right)$, and note that as $F$ is regular, $\phi$ is increasing, and hence $\max(\phi(v_1),\phi(v_2)) = \phi(\max\{v_1, v_2\})$.  Then by substituting for $\phi(\max\{v_1, v_2\})$ in the corollary, we see that it is equivalent to \[\mathbb{E}_{v_1, v_1 \sim F}\left[\left(1-\frac{1}{C(\alpha)}\right)\max\{v_1, v_2\} - \frac{1}{h(\max\{v_1, v_2\})} \; \biggr| \; \max\{v_1, v_2\} \geq t\right] \geq 0.\]  We rewrite this as \[\mathbb{E}_{v_1, v_1 \sim F}\left[\left(1-\alpha\right)\max\{v_1, v_2\} - \frac{1}{h(\max\{v_1, v_2\})} + \left(\alpha - \frac{1}{C(\alpha)}\right)\max\{v_1, v_2\} \; \biggr| \; \max\{v_1, v_2\} \geq t\right] \geq 0.\]  By the definition of $\alpha$-strong regularity, $\left(1-\alpha\right)\max\{v_1, v_2\} - \frac{1}{h(\max\{v_1, v_2\})}$ is always non-decreasing as a function of $\max\{v_1, v_2\}$. Additionally, we note that $1/C(\alpha) \leq \alpha$.  Therefore, conditioning on the event that $\max\{v_1, v_2\} \geq t$ only increases the expected value.
\end{proof}
}

\hide{
Finally, we have the following negative result for $\alpha$-SR regular distributions.  Note that in an MHR distribution, $H(2x) \geq 2H(x)$.

\begin{lem}\label{lem:double-arg}
For any constant $k > 0$ and $\alpha < 1$, there exists an $\alpha$-SR regular distribution such that $H(2x) < \frac{k+1}{k}H(x)$, for some $x$ when $\alpha < 1$.
\end{lem}

\begin{proof}
This lemma is equivalent to saying that for any positive constant $k$, there is an $x$ such that \[\int_0^{x} h(v)dv > k \int_x^{2x} h(v)dv.\]  Consider the following virtual valuation function $\phi$ for some distribution $F$.

\[\phi(v) = \begin{cases}
(2-\epsilon)(v-1) & \text{if }0 \leq v \leq 2 \\
v-\epsilon & \text{if }2 \leq v \leq 3 \\
(\alpha+\epsilon)(v-3)+3-\epsilon & \text{if }3 \leq v \leq 4 \\
\alpha(v-3)+3 & \text{if } 4 \leq x
\end{cases}.\]

Here, we consider only those $\epsilon$ in the range $(0, 1/2]$.  It can be checked that $\phi(v)$ is in fact the virtual valuation function of some $\alpha$-SR regular distribution.  Note that the reserve price is always $1$.  $\int_4^{8} h(v)dv$ is independent of $\epsilon$, while $\int_0^{4} h(v)dv$ is bounded below by $1/\epsilon$.  Therefore, for any $k$, we can choose $\epsilon$ so that $k < 1/\epsilon$, and we obtain a function as desired.

In the case $\alpha = 1$, the distribution does not extend beyond $4$.
\end{proof}
} 

==> sampling.tex <==

\section{Sample Complexity}
\label{sec:sampling}

Here we discuss the sample complexity of the mechanisms used in Theorem~\ref{thm-BGGm-w-sampling}. (The sample complexities of the mechanisms used in Theorems~\ref{thm:vcgl-samp},~\ref{thm:two-mech-samp} and~\ref{thm:lottery-samp} are deferred to the appendix.)
These mechanisms require knowledge of the distributions from which the valuations are drawn.  
% However, the distributions might not always be known.  Instead, we might have access to a certain number of samples from these distributions.  
We will show how to modify these mechanisms when the distributions are known approximately via samples.

 In~\cite{CR1}, this was done for the single-item auction by modifying the Myerson Auction.  Our mechanisms will follow the same format.  After obtaining the samples, we estimate the distributions, and use these in place of the actual distribution.  In particular, given $m$ samples, we first discard the $\lfloor \xi m \rfloor$ largest samples.  We let the emprical quantile of the $j$th largest sample $v_j$ be $\overline{q}(v_j) = 1-\overline{F}(v_j) = \frac{2j-1}{2m}$ and we let the empirical revenue curve be defined as $\overline{R}\left(\frac{2j-1}{2m}\right) = \frac{2j-1}{2m} v_j$, $\overline{R}(0) = \overline{R}(1) = 0$.  

We let $\CR$ be the convex hull of the actual revenue curve (which is convex for regular distributions).  Let $\overline{\CR}$ be the convex hull of the revenue curve, $\overline{\phi}$ the empirical virtual valuation function (i.e. the slope of $\overline{\CR}$), and $\overline{r}$ the empirical reserve price, i.e. the largest value such that $\overline{\phi}(\overline{r}) = 0. $ We will be overloading notation, writing both $\CR(q)$ and $\CR(v(q))$, and likewise for $\overline{\CR}$.

% \subsection{Preliminaries}

We start by stating results about the empirical revenue curve that will be used to modify mechanisms for the empirical setting.  The following is Lemma 6.2 from~\cite{CR1} and gives a lower bound on the accuracy of samples.
% Note that many of these results hold true even in the case of regular distributions.

\begin{lem}\label{empquantrange}
Let $F$ be a regular distribution (not necessarily strongly regular).  Suppose $m$ independent samples with values $v_1 \geq v_2 \geq \cdots \geq v_m$ are drawn from $F$.  Let $0 < \gamma, \xi < 1$ be given.  Let $t_j = \frac{2j-1}{2m}$.  Then for all $v \leq v_{\lfloor \xi m \rfloor}$ \[q(v) \in [\overline{q}(v)/(1+\gamma)^2, \overline{q}(v)(1+\gamma)^2]\] with probability at least $1-\delta$ if $\gamma \xi m \geq 4$, $(1+\gamma)^2 \leq \frac{3}{2}$, and $m \geq \frac{3}{\gamma^2(1+\gamma)\xi}\max\{\frac{\ln{3}}{\gamma}, \ln{\frac{3}{\delta}}\}$.
\end{lem}

We use Lemma~\ref{empquantrange} to prove the following result which shows that the value of the revenue curve at the empirical reserve price is a good approximation to the revenue at the actual reserve price.

\begin{lem}~\label{empreserve}
With probability at least $1-\delta$, \[\CR(\overline{r}) \geq \frac{1-\xi(1+\gamma)^2}{(1+\gamma)^4}\CR(r).\]
\end{lem}

\hide{The following corollary to the work in~\cite{CR1} shows that given an appropriate number of samples, the empirical reserve price is a $(1-\epsilon)$-optimal reserve price.  By this, we mean that $R(\overline{r}) \geq (1-\epsilon)R(r)$.  The proof follows the argument of Lemma $4.1$ from~\cite{DRY}.

\begin{cor}~\label{empreserve}Let $F$ be a regular distribution, and let $\gamma > 0, \xi = \frac{k}{m}$ for integers $k$ and $m$ be given be given.  Then the empirical reserve price $\overline{r}$ based on $m$ samples is a $(1-11\gamma)$-optimal reserve price with probability $1-\delta$ if $\gamma \xi m \geq 1$, $(1+\gamma)^2 \leq \frac{3}{2}$ and \[m \geq \frac{6}{\gamma^2(1+\gamma)\xi} \max\left\{\frac{\ln 3}{\gamma}, \ln{\frac{6}{\delta}}\right\}.\]
\end{cor}

We let $\mathcal{E}_{a}$ be the event that the outcome of Corollary~\ref{empreserve} holds.}

The following lemma from~\cite{CR1} describes the accuracy of the empirical revenue curves.

\begin{lem}\label{empquant}
Assume that the condition of Lemma~\ref{empquantrange} holds.  Then for all empirical quantiles $\overline{q}(\overline{r}) \geq \overline{q} \geq \xi$, \[\frac{1}{(1+\gamma)^3}\CR(\overline{q}(1+\gamma)^2) = \frac{1}{(1+\gamma)}\overline{q}v(\overline{q}(1+\gamma)^2) \leq \overline{\CR}(\overline{q}) \leq \overline{q}v\left(\frac{\overline{q}}{(1+\gamma)^2}\right) = (1+\gamma)^2\CR\left(\frac{\overline{q}}{(1+\gamma)^2}\right).\]  If $\overline{q}(\overline{r}) \leq \overline{q}$, then the right inequality holds, and the left inequality becomes \[\frac{1}{(1+\gamma)^3}\CR(\overline{q}(1+\gamma)^3) = \overline{q}v(\overline{q}(1+\gamma)^2) \leq \overline{\CR}(\overline{q}).\]
\end{lem}

\hide{
In order to use Lemma~\ref{empquant} to compare the empirical revenue curve with the actual one, we use the following lemma from~\cite{\CR1}.

\begin{lem}\label{valuequant}
Let $F$ be a regular distribution.  Let $q(r) \geq q_1 \geq q_2$, where $q(r)$ is the quantile of the reserve price for $F$.  Then $v(q_2) \leq \frac{q_1}{q_2}v(q_1)$.
\end{lem}

\begin{proof}
$\phi(q) \geq 0$ for $q \leq q(r)$, and consequently $R(q_1) \geq R(q_2)$.  $R(q_1) = q_1\cdot v(q_1)$ and $R(q_2) = q_2\cdot v(q_2)$.  Thus $q_1 \cdot v(q_1) \geq q_2\cdot v(q_2)$, and the result follows.
\end{proof}
}

\hide{
Using the above bound in Lemma~\ref{empquant} yields the following corollary.

\begin{cor}\label{empquantc}
Conditioned on $\mathcal{E}_a$, for all empirical quantiles $q(r) \geq \overline{q} \geq \xi$, \[\frac{1}{(1+\gamma)^2}\CR(\overline{q}) \leq \overline{\CR}(\overline{q}) \leq \CR(\overline{q})(1+\gamma)^2.\]
\end{cor}
}

\hide{
The following lemma, a slight modification of a claim in~\cite{CR1}, upper bounds the revenue curve for quantiles less than $q(r)$.  This will allow us to lower bound $q(\overline{r})$.

\skr{\begin{lem}\label{reserveb}
Let $F$ be an $\alpha$-SR regular distribution with monopoly price $r$.  For $q \leq q(r)$ and $0 < \alpha < 1$, \[\CR(q) \leq \CR(q(r)) \frac{1}{1-\alpha}\left(\frac{q}{q(r)}^{\alpha}-\alpha\frac{q}{q(r)}\right).\]
\end{lem}}
}

\hide{
\begin{lem}
Let $F$ be an $\alpha$-SR regular distribution with monopoly price $r$.  For $q_1 \leq q_2 \leq q(r)$ and $0 < \alpha < 1$, \[\CR(q_1) \leq \CR(q_2)\frac{1}{1-\alpha}\left(\frac{q_1}{q_2}\right)^{\alpha}.\]
\end{lem}

We note that the original lemma was proved in the case $q_2 = q(r)$.  However, the proof still holds in the case $q_2 \leq q(r)$.
}

\hide{
The following lemma lower bounds the quantile of the empirical reserve price in terms of the quantile of the actual reserve price.

\skr{\begin{lem}\label{reservequant}
Let $0 < \alpha \leq 1$, and let $F$ be an $\alpha$-SR regular distribution.  Then conditioned on $\mathcal{E}_a$, \[q(\overline{r}) \geq \left(1-\sqrt{\frac{8\gamma}{\alpha}}\right) q(r).\]
\end{lem}}

\begin{proof}
Assume for sake of contradiction that the statement of the lemma does not hold.  We show that this implies that $\overline{\CR}(r) \geq \overline{\CR}(\overline{r})$ which contradicts the choice of $\overline{r}$.

By Corollary~\ref{empquantc}, $\overline{\CR}(\overline{r}) \leq \CR(\overline{r})(1+\gamma)^2$.  To simplify the presentation, let $s = \sqrt{8\gamma/\alpha}$.  By our assumption on $g(\overline{r})$, we can apply Lemma~\ref{reserveb} to get a strict upper bound of \begin{align*}\CR(\overline{r})(1+\gamma)^2 &< \CR\left(\frac{q(r)}{1-s}\right)(1+\gamma)^2 \\
&\leq \CR(r)\frac{1}{1-\alpha}\left((1-s)^{\alpha}-\alpha(1-s)\right)(1+\gamma)^2 \numberthis \label{qbound}.\end{align*}  The Taylor approximation of $(1-s)^{\alpha}$ is $\sum_{i=0}^{\infty} \frac{(-1)^is^{i}\alpha(\alpha-1)\cdots(\alpha-i+1)}{i!}$. It follows that $(1-s)^{\alpha} \leq 1-\alpha s - (1-\alpha)\alpha s^2/2$.  Therefore~\eqref{qbound} is bounded above by \[\CR(r)\frac{1}{1-\alpha}\left(1-\alpha-\frac{\alpha s^2}{2}\right)(1+\gamma)^2 = \CR(r)\left(1-\frac{\alpha s^2}{2}(1+\gamma)^2\right) \numberthis \label{qboundtwo}.\]  Replacing $s$ with $\sqrt{8\gamma/\alpha}$ in~\eqref{qboundtwo} yields \[\CR(r)(1-4\gamma)(1+\gamma)^2 \leq \frac{1}{(1+\gamma)^2}\CR(r),\] as $1-4\gamma \leq 1/(1+\gamma)^4$.

%By our assumption, $q(\overline{r}) \leq q(r)$, and we can use Lemma~\ref{reserveb} to get a strict upper bound of \[\CR(r)(1+\gamma)^2\frac{1}{1-\alpha}\left(\left(\frac{1-\alpha}{(1+\gamma)^4}\right)^{1/\alpha}\right)^{\alpha} = \frac{\CR(r)}{(1+\gamma)^2}.\]  ]

By Corollary~\ref{empquantc} again, this is bounded above by $\overline{\CR}(r)$, reaching a contradiction.
\end{proof}
}

\hide{
\begin{proof}
We assume that the event $\mathcal{E}_a$ holds for all bidders, which it does with probability $1-k\delta$ by a union bound.  As in~\cite{CMM}, fix a bidder $i$, along with $(\mathbf{v_{-i}}, \mathbf{B})$ and consequently $T_i$.  Additionally, bidder $i$ only contributes to $\mathcal{R}^{\mathcal{M} \cap \mathcal{B}}$ if $v_i \geq T_i$. We consider two cases, $T_i \geq \overline{r}$ and $T_i \leq \overline{r}$.  The former case retains its proof in~\cite{CMM}.  In particular, \[\mathbb{E}_{v_i} [\mathcal{R}_i^{\mathcal{M} \cap \mathcal{B}}(\mathbf{v}, \mathbf{B}) | v_i \geq T_i] \leq \mathbb{E}_{v_i} [\mathcal{R}_i^{\mathcal{M^\mathcal{L}}}(\mathbf{v}, \mathbf{B}) | v_i \geq T_i]. \numberthis \label{three}\]  Here, $\mathcal{R}_i^{\mathcal{M}}$ is the revenue from bidder $i$ in mechanism $\mathcal{M}$.

In the case $T_i \leq \overline{r}$, as in Lemma 13 in~\cite{CMM}, \[\mathbb{E}_{v_i} [\mathcal{R}_i^{\mathcal{M} \cap \mathcal{B}}(\mathbf{v}, \mathbf{B}) | v_i \geq T_i] \leq \min\{r, B_i\}.\numberthis \label{one}\]  By Lemma 10 in~\cite{CMM}, if $v_i \geq \overline{r}$, then $\mathcal{R}_i^{\mathcal{M^\mathcal{L}}} \geq \min\{\overline{r}, B_i\}/3$.  This occurs with probability $1-F(\overline{r})$, and therefore \[\mathbb{E}_{v_i} [\mathcal{R}_i^{\mathcal{M^\mathcal{L}}}(\mathbf{v}, \mathbf{B}) | v_i \geq T_i] \geq \min\{\overline{r}, B_i\}(1-F(\overline{r}))/3.\]

In the case that $\min\{\overline{r}, B_i\} = \overline{r}$, by Corollary~\ref{empreserve}, the right-hand side is bounded below by $(1-11\gamma)(\min\{r, B_i\})(1-F(r))/3$.  In the case that $\min\{\overline{r}, B_i\} = B_i$, by Lemma~\ref{reservequant}, the right-hand side is bounded below by $\left(\frac{e-(e-1)(1+\gamma)^4}{e(1+\gamma)^4}\right)(1-F(r))/3$.  Therefore, in general \[\mathbb{E}_{v_i} [\mathcal{R}_i^{\mathcal{M^\mathcal{L}}}(\mathbf{v}, \mathbf{B}) | v_i \geq T_i] \geq \min\left\{\left(\frac{e-(e-1)(1+\gamma)^4}{e(1+\gamma)^4}\right), (1-11\gamma)\right\}(\min\{r, B_i\})(1-F(r))/3.\] By Lemma~\ref{reservebound}, this in turn becomes \[\mathcal{R}_i^{\mathcal{M^\mathcal{L}}}(\mathbf{v}, \mathbf{B}) | v_i \geq T_i] \geq \min\left\{\left(\frac{e-(e-1)(1+\gamma)^4}{e(1+\gamma)^4}\right), (1-11\gamma)\right\}(\min\{r, B_i\}) \alpha^{1/(1-\alpha)}/3. \numberthis \label{two}\] Combining~\eqref{one} and~\eqref{two} gives \begin{multline*}\mathbb{E}_{v_i} [\mathcal{R}_i^{\mathcal{M} \cap \mathcal{B}}(\mathbf{v}, \mathbf{B}) | v_i \geq T_i] \leq \\ 3\alpha^{-1/(1-\alpha)}\left(\min\left\{\left(\frac{e-(e-1)(1+\gamma)^4}{e(1+\gamma)^4}\right), (1-11\gamma)\right\}\right)^{-1} \mathbb{E}_{v_i} [\mathcal{R}_i^{\mathcal{M^\mathcal{L}}}(\mathbf{v}, \mathbf{B}) | v_i \geq T_i].\end{multline*}

We have just shown the above inequality  in the case $T_i \geq \overline{r}$; but by~\eqref{three} it also holds when $T_i \leq \overline{r}$.  Next, we note that when $v_i \leq T_i$, bidder $i$ does not contribute to $\mathcal{R}_i^{\mathcal{M} \cap \mathcal{B}}$, and consequently the conditioning can be ignored.  Taking the expectation over $(\mathbf{v_{-i}}, \mathbf{B})$ and summing over all $i$ yields the lemma.
\end{proof}
}

\subsection{Multi-item auctions with public budgets}

We now consider the mechanism in Theorem~\ref{lpmech}, first given in~\cite{CMM}. Here there is a set of bidders, a set of items, and a different distribution for the valuations for each (bidder, item) pair.  Each item can be assigned to at most one bidder, each bidder can receive only a specified number of items, and each bidder can spend no more than a pre-determined budget.

\hide{Because the valuations are chosen from a discrete set, Lemma~\ref{valuequant} and Corollary~\ref{empquantc} need not hold, and we rely on Lemma~\ref{empquant} instead.}

In addition, we add a point mass to the empirical distribution at $\overline{q}(\xi)$ so that $\overline{v}(q)$ and $\overline{q}(v)$ are defined for all quantiles greater than $\xi$ and all values less than $\overline{q}(\xi)$ respectively.

A key step in this mechanism is to solve the linear program LP2 below with coefficients derived from the distribution.  The optimal solution to LP2 yields a mechanism with the approximation guarantee stated in Theorem~\ref{lpmech}.  It is also the case that a feasible solution of LP2 achieving a solution with value $\rho \cdot OPT$ when substituted into a slight modification of the mechanism will yield an approximation factor of $\rho$ times the factor in Theorem~\ref{lpmech}.  As we only have access to samples of the distribution, we can only create an approximate form of LP2, which we name LP3, described below.  The main challenge is to show that a modification of an optimal solution to LP3 is feasible for LP2 and achieves a good approximation to the optimum of LP2. 

Notation: $\overline{f}$ and $\overline{\phi}$ are the approximations to $f$ and $\phi$ respectively, derived from the sample-based empirical distribution.  Additionally, $I$ is the set of bidders, $J$ is the set of items, $B_i$ is the budget of bider $i$, $n_i$ is the number of items bidder $i$ can obtain, and $R_{ij}$ is the support of the distribution $F_{ij}$ of the valuation of item $j$ by bidder $i$.  The virtual valuation function $\phi_{ij}$ is derived from $F_{ij}$.  Finally, $x_{ij}(r)$ is the variable in the linear program corresponding to $i \in I, j \in J$ and $r \in R_{ij}$.
%
\begin{alignat*}{3}
\text{Maximize } & \sum_{i \in I} \sum_{j \in J} \sum_{r \in R_{ij}} f_{ij}(r )\phi_{ij}(r) x_{ij}(r)\ \\
\text{Subject to: } ~&1. ~~ \sum_{j \in J} \sum_{r \in R_{ij}} f_{ij}(r)x_{ij}(r) \leq n_i & \quad & \forall i \in I \\
& 2. ~~ \sum_{j \in J} \sum_{r \in R_{ij}} f_{ij}(r)\phi_{ij}(r)x_{ij}(r) \leq B_i & \quad & \forall i \in I \tag{LP2}\\
& 3. ~~ \sum_{i \in I} \sum_{r \in R_{ij}} f_{ij}(r)x_{ij}(r) \leq 1 &\quad & \forall j \in J \\
& 4. ~~ 0 \leq x_{ij}(r) \leq 1 & \quad & \forall i \in I, j \in J, r \in R_{ij} \\
\end{alignat*}
%
\hide{\begin{alignat*}{2}
\text{Maximize } & \sum_{i \in I} \sum_{j \in J} \sum_{r \in R_{ij}} \overline{f}_{ij}(r)\overline{\phi}_{ij}(r) \overline{x}_{ij}(r)\ \\
\text{Subject to } & \sum_{j \in J} \sum_{r \in R_{ij}} \overline{f}_{ij}(r)\overline{x}_{ij}(r) \leq n_i/(1+\gamma)^2 & \quad & \forall i \in I \\
& \sum_{j \in J} \sum_{r \in R_{ij}} \overline{f}_{ij}(r)\overline{\phi}_{ij}(r)\overline{x}_{ij}(r) \leq B_i/(1+\gamma)^2 & \quad & \forall i \in I\tag{LP3} \\
& \sum_{i \in I} \sum_{r \in R_{ij}} \overline{f}_{ij}(r)\overline{x}_{ij}(r) \leq 1/(1+\gamma)^2 &\quad & \forall j \in J \\
& 0 \leq  \overline{x}_{ij}(r) \leq 1 & \quad & \forall i \in I, j \in J, r \in R_{ij}
\end{alignat*}}
%
LP3, given in the appendix, is obtained by replacing $f$ by $\overline{f}$, $\phi$ by $\overline{\phi}$, and $x$ by $\overline{x}$.

We will show that the optimal solution to LP3 is a good approximation to LP2.  We start by rewriting the above linear programs in a simpler format.  Let $x_{ij}^* = \sum_{r \in R_{ij}} f_{ij}(r ) x_{ij}(r)$; by Lemma 3.13 in~\cite{BGGM}, the optimum of LP2 is achieved when for some $L'$, $x_{ij}(r) = 0$ for $r < L'$, $x_{ij}(r) = 1$ for $r > L'$, and $0 \leq x_{ij}(L') \leq 1$ where $1 \leq L' \leq L$. Also, $\sum_{r \in R_{ij}} f_{ij}(r )\phi_{ij}(r) x_{ij}(r) = \CR_{ij}(x_{ij}^*)$.  We can define $\overline{x}_{ij}^*$ similarly; again $\sum_{r \in R_{ij}} \overline{f}_{ij}(r )\overline{\phi}_{ij}(r) \overline{x}_{ij}(r) = \overline{\CR}_{ij}(\overline{x}_{ij}^*)$.  These identities can be used to rewrite LP2 in terms of $x_{ij}^*$ rather than $x_{ij}(r)$, and LP3 in terms of $\overline{x}_{ij}^*$.  (The rewritten LPs are given in the appendix).
%
\hide{\begin{alignat*}{2}
\text{Maximize } & \sum_{i \in I} \sum_{j \in J} \CR_{ij}(x_{ij}^*)\ \\
\text{Subject to } & \sum_{j \in J} x_{ij}^* \leq n_i & \quad & \forall i \in I \\
& \sum_{j \in J} \CR_{ij}(x_{ij}^*) \leq B_i & \quad & \forall i \in I \tag{LP2} \\
& \sum_{i \in I} x_{ij}^* \leq 1 &\quad & \forall j \in J \\
& 0 \leq x_{ij}^* \leq 1 &\quad & \forall i \in I, j \in J
\end{alignat*}}
\hide{
\begin{alignat*}{2}
\text{Maximize } & \sum_{i \in I} \sum_{j \in J} \overline{\CR}_{ij}(\overline{x}_{ij}^*)\ \\
\text{Subject to } & \sum_{j \in J} \overline{x}_{ij}^* \leq n_i & \quad & \forall i \in I \\
& \sum_{j \in J} \overline{\CR}_{ij}(\overline{x}_{ij}^*) \leq B_i & \quad & \forall i \in I \tag{LP3} \\
& \sum_{i \in I} \overline{x}_{ij}^* \leq 1 &\quad & \forall j \in J \\
& 0 \leq \overline{x}_{ij}^* \leq 1 &\quad & \forall i \in I, j \in J
\end{alignat*}
}

Finally, we note that in the optimal solution of both LP2 and LP3, $x_{ij}^*$ and $\overline{x}_{ij}^*$ are no larger than the reserve price quantiles of the distributions $F_{ij}$ and $\overline{F}_{ij}$ respectively, for all $i$ and $j$.  To see this, consider any $x_{ij}^*$ for which this is not the case.  Because $\CR_{ij}$ is convex and $\CR(0) = \CR(1) = 0$, there is another point $y$ such that $\CR(x_{ij}^*) = \CR(y)$, but with $y < q(r)$.  Therefore, we can replace $x_{ij}^*$ with $y$, without changing the value of the objective function and continuing to satisfy all the constraints.  This is the case for both $x_{ij}^*$ in LP2 and $\overline{x}_{ij}^*$ in LP3.

As described in~\cite{BGGM}, the distributions $F_{ij}$ are truncated so that the support does not include any value greater than $B_{i}$.  Therefore $\CR_{ij}(q) \leq B_i q$ for all $i$ and $j$, and quantiles $q$.  This bound also holds for $\overline{\CR}_{ij}(q)$.  To see this, let the point $(q, \overline{\CR}_{ij}(q))$ lie on the line segment from $(\frac{2k_1-1}{m}, \frac{2k_1-1}{m}v_{k_1})$ to $(\frac{2k_2-1}{m}, \frac{2k_2-1}{m}v_{k_2})$.  If $v_{k_1} = v_{k_2} = B_i$ then $\overline{\CR}_{ij}(q) = qB_i$, but if $v_{k_1}$ or $v_{k_2}$ were any smaller, the value of $\overline{\CR}_{ij}(q)$ would also be smaller.  

\hide{This fact will be used in the following lemma which shows that the optimum of LP3 is close to that of LP2.}

\hide{\begin{lem}
Let the optimal solutions of LP2 and LP3 be $x$ and $\overline{x}$, respectively.  Let \[V_2 = \sum_{i \in I} \sum_{j \in J} \CR_{ij}(x_{ij}^*) \text{ and } V_3 = \sum_{i \in I} \sum_{j \in J} \CR_{ij}(\overline{x}_{ij}^*/(1+\gamma)^2).\]  Then with probability $1-|I||J|\delta$, \[V_2+(1+\gamma)^2|J| \sum_{i \in I} B_i \xi \geq V_3 \geq \frac{1}{(1+\gamma)^8}V_2 - \left(1+\frac{1}{(1+\gamma)^8}\right)|J|\sum_{i \in I} B_i \xi,\] if the empirical distribution is determined by $m \geq \frac{6(1+\gamma)}{\gamma^2\xi} \max\{\frac{\ln{3}}{\gamma}, \ln\frac{3}{\delta}\}$ samples.
\end{lem}}
\hide{
\begin{proof}
We assume that the event $\mathcal{E}_a$ occurs for all distributions $F_{ij}$, which it does with probability $1-|I||J|\delta$.  We start with the left inequality.  Consider the optimal assignment to LP3, $\overline{x}_{ij}^*$, and assume for the moment that $\overline{x}_{ij}^* \geq \xi(1+\gamma)^4$.  Consider the variables $\overline{y}_{ij}^*$ defined by $\overline{y}_{ij}^* = \overline{x}_{ij}^*/(1+\gamma)^2$.  Thus $\overline{y}_{ij}^* \geq \xi(1+\gamma)^2$.

Note that by Lemma 3.13 in~\cite{BGGM}, we can write $\overline{y}_{ij}^*$ as \[\overline{y}_{ij}^* = \sum_{r \in R_{ij}} f_{ij}(r ) \overline{y}_{ij}(r),\] where $0 \leq \overline{y}_{ij}(r) \leq 1$ and satisfy \[\sum_{r \in R_{ij}} f_{ij}(r )\phi_{ij}(r) \overline{y}_{ij}(r) = \CR_{ij}(\overline{y}_{ij}^*).\]

We show that the assignment $\overline{y}^*$ satisfies the constraints of LP2.  The first and third constraints of LP2 hold, as \[\sum_{j \in J} \overline{y}_{ij}^* \leq \frac{1}{(1+\gamma)^2}\sum_{j \in J} \overline{x}_{ij}^* \leq n_i\] and \[\sum_{i \in I} \overline{y}_{ij}^* \leq \frac{1}{(1+\gamma)^2}\sum_{i \in I} \overline{x}_{ij}^* \leq 1\] as desired.

Now consider the second constraint.  By Lemma~\ref{empquant}, as $\overline{y}_{ij}^* \geq \xi(1+\gamma)^2$, $\CR(\overline{y}_{ij}^*) \leq (1+\gamma)^2 \overline{\CR}(\overline{y}_{ij}^*/(1+\gamma)^2)$.  Because the empirical reserve price $\overline{r}$ is greater than $\overline{x}_{ij}^*$ which in turn is greater than $\overline{y}_{ij}^*/(1+\gamma)^2$, it is also true that $\overline{\CR}(\overline{y}_{ij}^*/(1+\gamma)^2) \leq \overline{\CR}(\overline{x}_{ij}^*)$.  Therefore for each $i$,
%
\begin{align*}
\sum_{j \in J} \CR(\overline{y}_{ij}^*) &\leq (1+\gamma)^2 \sum_{j \in J} \overline{\CR}(\overline{y}_{ij}^*/(1+\gamma)^2) \\
&\leq (1+\gamma)^2 \sum_{j \in J} \overline{\CR}(\overline{x}_{ij}^*) \\
&\leq (1+\gamma)^2 B_i/(1+\gamma)^2 \\
&= B_i \end{align*} and the second constraint is satisfied.

If we do not make assumptions on the values of $\overline{y}_{ij}^*$, then the first and third constraints of LP2 still hold, but the second might not be satisfied.  If we decrease the value of all $\overline{y}_{ij}^*$ with values less than $\xi(1+\gamma)^2$ to zero, then the constraints of LP2 will all be satisfied as $\CR(\overline{y}_{ij}^*) = 0$ in this case.  However, this might decrease the value of the objective function.  Let $S$ be the set of all $(i, j)$ pairs such that $\overline{y}_{ij}^* < \xi(1+\gamma)^2$.  Then \begin{align*}
V_2 &\geq \sum_{(i, j) \in I \times J \backslash S} \CR_{ij}(\overline{y}_{ij}^*) \\
&= \sum_{i \in I} \sum_{j \in J} \CR_{ij}(\overline{y}_{ij}^*) - \sum_{(i, j) \in S} \CR_{ij}(\overline{y}_{ij}^*) \\
&\geq \sum_{i \in I} \sum_{j \in J} \CR_{ij}(\overline{y}_{ij}^*) - \sum_{(i, j) \in S} B_i\overline{y}_{ij}^* \\
&\geq V_3 -(1+\gamma)^2 |J|\sum_{i\in I}B_i\xi.\end{align*}  The second inequality follows from the fact that $\CR_{ij}(q) \leq B_iq$.  The third inequality uses the fact that $(i, j) \in S$ only if $\overline{y}_{ij}^* < \xi(1+\gamma)^2$.  Therefore, \[V_2+(1+\gamma)^2|J| \sum_{i \in I} B_i \xi \geq V_3\] as desired.

Now we prove the right inequality in the lemma.  Consider the optimal assignment to LP2, $x^*$.  Assume for the moment that $x_{ij}^* \geq \xi(1+\gamma)^2$ for all pairs $i$ and $j$. We start by defining the variables $z_{ij}^*$ as follows: \[z_{ij}^* =  x_{ij}^*/(1+\gamma)^2.\] Again, by Lemma 3.13 in~\cite{BGGM}, we can write $z_{ij}^*$ as \[z_{ij}^* = \sum_{r \in R_{ij}} \overline{f}_{ij}(r ) z_{ij}(r),\] where $0 \leq z_{ij}(r) \leq 1$ satisfy \[\sum_{r \in R_{ij}} \overline{f}_{ij}(r )\overline{\phi}_{ij}(r) z_{ij}(r) = \overline{\CR}_{ij}(z_{ij}^*).\]  We let $y_{ij}(r) = z_{ij}(r)/(1+\gamma)^4$; thus \[\sum_{r \in R_{ij}} \overline{f}_{ij}(r )\overline{\phi}_{ij}(r) y_{ij}(r) = \overline{\CR}_{ij}(z_{ij}^*)/(1+\gamma)^4.\]

We show that the assignment $y$ satisfies the constraints of LP3.  To do this, we use the original form of the linear program. The first constraint holds, as \begin{align*}\sum_{j \in J} \sum_{r \in R_{ij}} \overline{f}_{ij}(r ) y_{ij}(r) &= \frac{1}{(1+\gamma)^4}\sum_{j \in J} z_{ij}^* \\
&\leq \frac{1}{(1+\gamma)^6}\sum_{j \in J} x_{ij}^* \\
&\leq n_i/(1+\gamma)^6. \end{align*}  The third constraint also holds, as  \begin{align*}\sum_{i \in I} \sum_{r \in R_{ij}} \overline{f}_{ij}(r ) y_{ij}(r) &= \frac{1}{(1+\gamma)^4}\sum_{i \in I} z_{ij}^* \\
 &\leq \frac{1}{(1+\gamma)^6}\sum_{i \in I} x_{ij}^* \\
&\leq 1/(1+\gamma)^6. \end{align*}  Finally note that $\overline{\CR}_{ij}(z_{ij}^*)$ is bounded above by $\CR_{ij}(x_{ij}^*)(1+\gamma)^2$.  By Lemma~\ref{empquant}, $\overline{\CR}_{ij}(z_{ij}^*)$ is bounded above by $(1+\gamma)^2\CR(x_{ij}^*/(1+\gamma)^4)$.  However, because $r_{ij} \geq x_{ij}^* \geq x_{ij}^*/(1+\gamma)^4$, we have $\CR(x_{ij}^*/(1+\gamma)^4) \leq \CR(x_{ij}^*)$. Therefore, the second constraint holds, as for every $i,$
\begin{align*}
\sum_{j \in J} \sum_{r \in R_{ij}} \overline{f}_{ij}(r )\overline{\phi}_{ij}(r) y_{ij}(r) &= \frac{1}{(1+\gamma)^4} \sum_{j \in J} \overline{\CR}_{ij}(z_{ij}^*) \\
&\leq \frac{1}{(1+\gamma)^4}\sum_{j \in J} \CR_{ij}(x_{ij}^*)(1+\gamma)^2\\
&\leq B_i/(1+\gamma)^2.
\end{align*}
%
If we do not make any assumptions on $x_{ij}^*$ in the optimal assignment to LP2, then the constraints of LP3 will still be satisfied after the replacement and scaling.  In the case that $x_{ij}^* < \xi(1+\gamma)^2$, we let $z_{ij}^*$ and all $y_{ij}(r)$ be $0$.  Because $\CR_{ij}(0) = 0$,  the constraints remain satisfied.  Let $T$ be the set of all $(i, j)$ pairs such that $x_{ij}^* < \xi(1+\gamma)^2$.  As before, let $\overline{x}$ be the optimal solution to LP3 and let $S'$ be the set of all $(i, j)$ pairs such that $\overline{x}_{ij}^* \leq \xi$. Then by Lemma~\ref{empquant} and the fact that $\CR_{ij}(q) \leq B_iq$,
\begin{align*} V_3 &=  \sum_{i \in I} \sum_{j \in J} \CR_{ij}(\overline{x}_{ij}^*/(1+\gamma)^2) \\
&\geq \sum_{(i,j)\in (I \times J) / S'} \CR_{ij}(\overline{x}_{ij}^*/(1+\gamma)^2) \\
&\geq \sum_{i \in I} \sum_{j \in J} \overline{\CR}_{ij}(\overline{x}_{ij}^*)/(1+\gamma)^2 - \sum_{(i, j) \in S'} B_i\xi \\
&= \frac{1}{(1+\gamma)^2}\sum_{i \in I} \sum_{j \in J} \sum_{r \in R_{ij}} \overline{f}_{ij}(r )\overline{\phi}_{ij}(r) \overline{x}_{ij}(r) - \sum_{(i, j) \in S'} B_i\xi.\end{align*}
%
Because $y$ satisfies the constraints of LP3, the value of the objective function of LP3 with $y$ substituted is a lower bound to the value of the objective of LP3 with the optimal assignment $\overline{x}$.  Therefore we can lower bound the above by \[\frac{1}{(1+\gamma)^2}\sum_{i \in I} \sum_{j \in J} \sum_{r \in R_{ij}} \overline{f}_{ij}(r )\overline{\phi}_{ij}(r) y_{ij}(r) - \sum_{(i, j) \in S'} B_i\xi.\] Using the identity $\sum_{r \in R_{ij}} \overline{f}_{ij}(r )\overline{\phi}_{ij}(r) y_{ij}(r) = \overline{\CR}_{ij}(z_{ij}^*)/(1+\gamma)^4$, we can rewrite this as \[\frac{1}{(1+\gamma)^6}\sum_{i \in I}\sum_{j \in J}\overline{\CR}_{ij}(z_{ij}^*) - \sum_{(i, j) \in S'} B_i\xi \geq \frac{1}{(1+\gamma)^6}\sum_{(i, j) \in (I\times J) / T} \overline{\CR}_{ij}(z_{ij}^*) - \sum_{(i, j) \in S'} B_i\xi\] Finally, by Lemma~\ref{empquant} and the fact that $\CR_{ij}(q) \leq B_iq$, the above is lower bounded by\begin{multline*}\frac{1}{(1+\gamma)^8}\sum_{(i, j) \in (I\times J) / T} \CR_{ij}(x_{ij}^*)+\frac{1}{(1+\gamma)^8}\sum_{(i, j) \in T}\left( \CR_{ij}(x_{ij}^*)-B_i\xi\right) - \sum_{(i, j) \in S'} B_i\xi \geq \\ V_2/(1+\gamma)^8 - |J|\sum_{i \in I} B_i\xi\left(1+\frac{1}{(1+\gamma)^8}\right).\end{multline*}
\end{proof}
}

We modify the mechanism given in~\cite{BGGM}.  In particular, we replace the step that solves LP2 with a step to solve LP3 to obtain the solution $\overline{x}_{ij}^*$.  We then construct $\overline{z}_{ij}^* = \max\{\overline{x}_{ij}^*, \xi(1+\gamma)^2\}$, and use $\overline{v}(\overline{z}_{ij}^*)$ in the mechanism.  Additionally, instead of offering each item to each bidder with probability $1/4$, we do so with probability $(1-c\xi)/(4(1+\gamma)^2)$ where $c = \max\{|I|, |J|\}(1+\gamma)^4$.

%As we will show, $\overline{y}_{ij}(r) = (1-c\xi)\overline{z}_{ij}(r)$ satisfies LP2 and further achieves a good approximation of the optimum, the value achieved by $x_{ij}^*$.

Recall that, as proved in Lemma 3.13 in~\cite{BGGM}, $\overline{v}(\overline{z}_{ij}^*)$ can be written as $\overline{w}_{ij}^*\overline{r}_{ij}+(1-\overline{w}_{ij}^*)(\overline{r}_{ij}+1)$ where $\overline{r}_{ij} \in R_{ij}$ and $0 \leq \overline{w} \leq 1$.  Additionally, $\overline{\CR}(\overline{z}_{ij}^*)=\overline{w}_{ij}^*\overline{\CR}(r_{ij})+(1-\overline{w}_{ij}^*)\overline{\CR}(r_{ij}+1)$.  The $\overline{r}_{ij}$ and $\overline{w}_{ij}^*$ will be used in the mechanism given below in Figure 1.


\begin{figure}{\parbox{\textwidth}{
\begin{enumerate}
\item Solve LP3, and let $\overline{z}_{ij}^*$ be as defined previously.

\item Process the bidders in term in some fixed, but arbitrary order.

\item For each $(i, j)$ let $\widetilde{r}_{ij}$ be $\overline{r}_{ij}$ with probability $\overline{w}_{ij}^*$ and $\overline{r}_{ij}+1$ with probability $1-\overline{w}_{ij}^*$, where $\overline{r}_{ij}$ and $\overline{w}_{ij}^*$ are as defined previously.

\item For each $(i, j)$ let $Y_{ij}$ be a $0/1$ random variable so that $Y_{ij} = 1$ with probability $(1-c\xi)/(4(1+\gamma)^2)$ and $Y_{ij} = 0$ otherwise.

\item Offer each bidder $i$ all items $j$ with $Y_{ij} = 1$ that have not already been bought, at price $\tilde{r}_{ij}$.
\end{enumerate}
}}
\caption{Posted-Price Mechanism}\end{figure}

\hide{In particular, we do this for a slight modification to the optimal solution $\overline{x}_{ij}^*$ of LP3.  Let $\overline{z}_{ij}^* = \max\{\overline{x}_{ij}^*, \xi(1+\gamma)^4\}/(1+\gamma)^2$.  By Lemma 3.13 in~\cite{BGGM}, as $\overline{z}_{ij}^*$ is a quantile, we can write it as $\overline{z}_{ij}^* = \sum_{r \in R_{ij}} f_{ij}(r ) \overline{z}_{ij}(r)$.  Note that the original distribution is used, and not the empirical distribution.  Then we let the modification be $\overline{y}_{ij}(r) = \frac{1-c\xi}{(1+\gamma)^2}\overline{z}_{ij}(r)$ where $c = \max\{|I|, |J|\}(1+\gamma)^4$.}

Consider the quantile $q(\overline{v}(\overline{z}_{ij}^*))$.  This is the probability that bidder $i$'s valuation of item $j$ is at least $\widetilde{r}_{ij}$. By Lemma 3.13 in~\cite{BGGM}, it can be written as $\sum_{r \in R_{ij}} f_{ij}(r ) q(\overline{v}(\overline{z}_{ij}^*))(r)$.  Note that the original distribution is used, and not the empirical distribution.  Then consider the variables $\overline{y}_{ij}(r)$ defined as $\overline{y}_{ij}(r) = \frac{1-c\xi}{(1+\gamma)^2}q(\overline{v}(\overline{z}_{ij}^*))(r)$ where $c = \max\{|I|, |J|\}(1+\gamma)^4$.  The following lemma shows that $\overline{y}_{ij}$ satisfies LP2.  This will be used to show that the mechanism in Figure 1 satisfies the allocation bounds with constant probability.


%\skr{We first show that that the objective function of LP2 on the variables $\overline{y}_{ij}(r)$ achieves a value that is a multiplicative approximation to the value on the optimal solution.  }

\begin{lem}\label{lp2constraint}
The $\overline{y}_{ij}$ described above satisfy the constraints of LP2 with probability $1-|I|J|\delta$.  
\end{lem}
\begin{proof}
Assume that the conditions of Lemma~\ref{empquantrange} hold, which they do with probability $1-|I||J|\delta$.  Consider the second constraint.  By Lemma~\ref{empquantrange}, as $\overline{z}_{ij}^* \geq \xi(1+\gamma)^2$, \[\CR_{ij}(q(\overline{v}(\overline{z}_{ij}^*))) = q(\overline{v}(\overline{z}_{ij}^*))\overline{v}(\overline{z}_{ij}^*) \leq (1+\gamma)^2\overline{z}_{ij}^*\overline{v}(\overline{z}_{ij}^*) = (1+\gamma)^2 \overline{\CR}_{ij}(\overline{z}_{ij}^*)\numberthis \label{crbound}.\]  Additionally, if $\overline{z}_{ij}^* = \xi(1+\gamma)^2$, then $\CR_{ij}(\overline{z}_{ij}^*) \leq B_{i}\xi(1+\gamma)^2$.  Otherwise, $\overline{z}_{ij}^* = \overline{x}_{ij}^*$,  and $\overline{\CR}_{ij}(\overline{z}_{ij}^*) = \overline{\CR}_{ij}(\overline{x}_{ij}^*)$.  Therefore for each $i$, \begin{align*}\sum_{j \in J} \sum_{r \in R_{ij}} f_{ij}(r)\phi_{ij}(r)\overline{y}_{ij}(r) & = \frac{1-c\xi}{(1+\gamma)^2}\sum_{j \in J} \CR_{ij}(q(\overline{v}(\overline{z}_{ij}^*))) \\
&\leq ({1-c\xi}) \sum_{j \in J} \overline{\CR}_{ij}(\overline{z}_{ij}^*) \tag{by~\eqref{crbound}}\\
&\leq ({1-c\xi}) \sum_{j \in J} \left(\overline{\CR}_{ij}(\overline{x}_{ij}^*)+B_{i}\xi{(1+\gamma)^2}\right)\\
&\leq (1-|J|(1+\gamma)^4\xi)B_i+|J|B_i(1+\gamma)^2\xi \\
&\leq B_i \end{align*} and the second constraint is satisfied.

The proofs that the first and third constraints hold are similar and are deferred to the appendix.
\end{proof}

We also show that the value of the optimization function of LP2 on the solution $\overline{y}_{ij}$ is close to its value on the optimal solution $x_{ij}^*$.

\begin{lem}\label{lp3}
Let $\overline{y}_{ij}$ be as described above, let $x_{ij}^*$ be the optimal solution of LP2, and define \[V_2 = \sum_{i \in I} \sum_{j \in J} \CR_{ij}(x_{ij}^*) \text{, and } V_3 = \sum_{i \in I} \sum_{j \in J} \sum_{r \in R_{ij}} f_{ij}(r ) \overline{\phi}_{ij}(r)\overline{y}_{ij}(r).\]  Then with probability $1-|I||J|\delta$, $V_3 \geq \frac{(1-c\xi)(1-c'\xi)(1-\xi(1+\gamma)^3)^2}{(1+\gamma)^9} V_2,$ where $c = \max\{|I|, |J|\}(1+\gamma)^4$, $c' = \max\{|I|, |J|\}(1+\gamma)^2$, and the empirical distribution is determined by $m \geq \frac{6(1+\gamma)}{\gamma^2\xi} \max\{\frac{\ln{3}}{\gamma}, \ln\frac{3}{\delta}\}$ samples, with $\gamma \xi m \geq 4$ and $(1+\gamma)^2 \leq \frac{3}{2}$.
\end{lem}

\begin{proof}
Assume that the conditions of Lemma~\ref{empquantrange} hold, which they do with probability $1-|I||J|\delta$.  Consider the optimal assignment to LP2, $x_{ij}^*$.  We show that a slight modification to $x_{ij}^*$ satisfies the conditions of LP3, and will use this to bound $V_3$ from below.  Let $z^*_{ij} = \max\{x^*_{ij}, (1+\gamma)^2\xi\}/(1+\gamma)^2$ if $z^*_{ij} \leq \overline{q}(\overline{r})$ and $\max\{x^*_{ij}, (1+\gamma)^3\xi\}/(1+\gamma)^3$ otherwise.  For convenience, let $e_{ij}$ satisfy $z^*_{ij} = \max\{x^*_{ij}, (1+\gamma)^{e_{ij}}\xi\}/(1+\gamma)^{e_{ij}}$.  By Lemma 3.13 in~\cite{BGGM}, we can write $z_{ij}^*$ as $z_{ij}^* = \sum_{r \in R_{ij}} \overline{f}_{ij}(r ) z_{ij}(r)$, and we let $y_{ij}(r) = \frac{1-c'\xi}{(1+\gamma)^2}z_{ij}(r)$ where $c' = \max\{|I|, |J|\}(1+\gamma)^2$.  We show that $y_{ij}$ satisfies the constraints of LP3 in the appendix, with an argument similar to that of Lemma~\ref{lp2constraint}.

We now bound $V_3$ from below.  Using the identity $\sum_{r \in R_{ij}} f_{ij}(r)\phi_{ij}(r)\overline{y}_{ij}(r) = \frac{1-c\xi}{(1+\gamma)^2} \CR_{ij}(q(\overline{v}(\overline{z}_{ij}^*)))$ and applying Lemma~\ref{empquantrange} to $q(\overline{v}(\overline{z}_{ij}^*))$, it follows that\begin{align*}
V_3 =  \sum_{i \in I} \sum_{j \in J} \sum_{r \in R_{ij}} f_{ij}(r )\phi_{ij}(r) \overline{y}_{ij}(r)
&= \frac{1-c\xi}{(1+\gamma)^2}\sum_{i \in I} \sum_{j \in J} \CR_{ij}(q(\overline{v}(\overline{z}_{ij}^*))) \\
&\geq \frac{1-c\xi}{(1+\gamma)^4}\sum_{i \in I} \sum_{j \in J} \overline{\CR}_{ij}(\overline{z}^*_{ij}) \numberthis \label{vthreebound}\end{align*}  We next compare $\overline{\CR}_{ij}(\overline{z}^*_{ij})$ to $\overline{\CR}_{ij}(\overline{x}_{ij}^*)$.  If $\overline{z}^*_{ij} = \overline{x}^*_{ij}$, then the two are equal.  Otherwise, $\overline{z}^*_{ij} = \xi(1+\gamma)^2$ and it follows from the convexity of $\overline{\CR}$ that $(1-\xi(1+\gamma)^2)\overline{\CR}_{ij}(\overline{x}^*_{ij}) \leq \overline{\CR}_{ij}(\overline{z}_{ij}^*)$.  Therefore, we can lower bound~\eqref{vthreebound} and hence $V_3$ by 
\[V_3 \geq \frac{(1-c\xi)(1-\xi(1+\gamma)^2)}{(1+\gamma)^4}\sum_{i \in I} \sum_{j \in J} \overline{\CR}_{ij}(\overline{x}^*_{ij}).\] Because $\overline{x}_{ij}^*$ is the optimal solution to LP3, it follows that $\sum_{i \in I} \sum_{j \in J}\overline{\CR}_{ij}(\overline{x}_{ij}) \geq \sum_{i \in I} \sum_{j \in J}\sum_{r \in R_{ij}} \overline{f}_{ij}(r)\overline{\phi}_{ij}(r) y_{ij}(r)$, yielding a lower bound on $V_3$ of
\[V_3 \geq \frac{(1-c\xi)(1-\xi(1+\gamma)^{2})}{(1+\gamma)^{4}}\sum_{i \in I} \sum_{j \in J} \sum_{r \in R_{ij}} \overline{f}_{ij}(r)\overline{\phi}_{ij}(r) y_{ij}(r).\]  Using the identity $\sum_{r \in R_{ij}} \overline{f}_{ij}(r )\overline{\phi}_{ij}(r) y_{ij}(r) = \frac{1-c'\xi}{(1+\gamma)^2}\overline{\CR}_{ij}(z_{ij}^*)$, yields \[V_3 \geq \frac{(1-c\xi)(1-c'\xi)(1-\xi(1+\gamma)^{2})}{(1+\gamma)^{6}}\sum_{i \in I} \sum_{j \in J} \overline{\CR}_{ij}(z^*_{ij}).\]  We apply Lemma~\ref{empquant} to obtain a lower bound of \[V_3 \geq \frac{(1-c\xi)(1-c'\xi)(1-\xi(1+\gamma)^{2})}{(1+\gamma)^{9}}\sum_{i \in I} \sum_{j \in J} \CR_{ij}(z_{ij}(r)(1+\gamma)^{e_{ij}}).\] Similarly as before, because $(1-\xi(1+\gamma)^3)\CR(x_{ij}^*) \leq \CR(z^*_{ij}(1+\gamma)^{e_{ij}})$ we lower bound the above by
\begin{align*}V_3 &\geq \frac{(1-c\xi)(1-c'\xi)(1-\xi(1+\gamma)^2)(1-\xi(1+\gamma)^3)}{(1+\gamma)^{9}}\sum_{i \in I} \sum_{j \in J} \CR_{ij}(x^*_{ij}) \\
&= \frac{(1-c\xi)(1-c'\xi)(1-\xi(1+\gamma)^2)(1-\xi(1+\gamma)^3)}{(1+\gamma)^{9}} V_2.
\end{align*}
\end{proof}

%The revenue guarantee of Theorem~\ref{thm-BGGm-w-sampling} follows from this and the fact that the mechanism in Figure~1 allocates with probabilities at least $\overline{y}_{ij}/4$.}


\hide{Because this is the only step of the mechanism described in~\cite{BGGM} that relies on knowledge of the distribution, Lemma~\ref{lp3} is enough to show that the empirical mechanism achieves a good approximation.  In particular, we replace the step that solves LP2 with a step to solve LP3, and divide all the variables by a $(1+\gamma)^2$ factor.}


\begin{thm}
\label{thm-BGGm-w-sampling}
The empirical posted-price mechanism in Figure 1 gives an approximation to the optimal truthful-in-expectation Bayesian incentive-compatible mechanism with a multiplicative error of \[\frac{192}{\alpha}\left(\frac{2-\alpha}{\alpha}\right)^{1/(1-\alpha)}\frac{(1-c\xi)(1-c'\xi)(1-\xi(1+\gamma)^{3})^2}{(1+\gamma)^{9}}(1-|I||J|\delta),\] given $m \geq \frac{6(1+\gamma)}{\gamma^2\xi} \max\{\frac{\ln{3}}{\gamma}, \ln\frac{3}{\delta}\}$ samples if $\gamma \xi m \geq 4$ and $(1+\gamma)^2 \leq \frac{3}{2}$.
\end{thm}
\begin{proof}
Using the same proof as in Theorem 3.13 in~\cite{BGGM}, we can show that the mechanism in Figure 1 allocates item $j$ to bidder $i$ with probability $\frac{1}{6} \cdot \frac{\overline{y}_{ij}^*}{4}.$  This follows from the fact that $\overline{y}_{ij}$ satisfies the constraints of LP2, as stated in Lemma~\ref{lp2constraint}.  By Lemma~\ref{lp3}, the objective function of LP2 at $\overline{y}_{ij}$ is close to the optimum $V_2$, with probability $1-|I||J|\delta.$

Finally, $\frac{1}{24}V_2$, the revenue guaranteed by Theorem~\ref{lpmech}, is a $\frac{192} {\alpha} \left( \frac {2 - \alpha} {\alpha} \right)^{1/(1 - \alpha)}$ approximation to the revenue of the optimal mechanism.  By the same analysis, the mechanism in Figure 1 yields revenue $\frac{1}{24}V_3$, yielding the desired bound.
\end{proof}
